PAREDA: A Multi-Accent Speech Dataset of Natural Language Processing Research Discussions

While modern Automatic Speech Recognition (ASR) systems achieve high accuracy on benchmark corpora, their performance often degrades when there is real-world variability. This work focuses on variability arising due to accented, spontaneous, and domain-specific speech. In particular, we introduce PAper REading DAtaset (PAREDA), a first-of-its-kind multi-accent speech dataset consisting of discussions on academic Natural Language Processing (NLP) papers between speakers with Australian, Indian-English, and Chinese English accents. Each session elicits a spontaneous monologue (a summary of a paper's abstract) and a non-monologue (a question-and-answer session between participants), resulting in a corpus rich with technical jargon and conversational phenomena. We evaluate the performance of SOTA ASR models on PAREDA, analysing the impact of accent mixing and increased speech rate. Our results show that, in the zero-shot setting, models perform worse, confirming the dataset's challenging nature. However, fine-tuning on PAREDA significantly reduces the Word Error Rate (WER), demonstrating that our dataset captures linguistic characteristics often missing from existing corpora. PAREDA serves as a valuable new resource for building and evaluating more robust and inclusive ASR systems for specialised, real-world applications.

==> sections/06-ethics.tex <==
\section*{Limitations}


% This simplification may partly explain the high sarcasm detection error for en-IN (46\%), where regional variation is especially pronounced. While BESSTIE pushes SOTA in dataset availability, capturing fine-grained sub-varieties is a valuable direction for future work.

% Our experiments do not exhaustively explore all potential architectures (encoder-decoder models) or training methodologies (other fine-tuning methods). Although we fine-tuned and benchmarked popular models, performance variability may arise from factors like pre-training data distribution, model size, and the training regime. Furthermore, cross-variety generalization remains an open challenge, as our analysis suggests models fine-tuned on one variety do not always generalize well to another, highlighting limitations in model adaptability.er

\section*{Ethical Considerations}

\section*{Acknowledgements}


% \begin{itemize}
%     \item Ethics approval. (only mention we have approval. no number at the anon review stage.)
%     \item No attempt to de-identify since no context.
%     \item Publicly available posts accessible through official APIs.
%     \item Data sharing policy?
% \end{itemize}

==> sections/backup_discussion.tex <==
\section{Discussion}
The benchmark results show the need to further probe into factors influencing model performances. These factors include tasks, training data and model properties. 
% Table~\ref{tab:arch} describes the model performances (reporting \f), grouped based on their properties. 

% \begin{table*}[t!]
%     \centering
%     \begin{adjustbox}{width=1.0\linewidth,center}
%     \renewcommand{\arraystretch}{1.1}
%     \setlength{\cmidrulekern}{0.25em}    
%     \begin{tabular}{cccc}
%     \toprule
%     \multirow{2}{4em}{\centering Locale} & \multicolumn{3}{c}{Domain-Task}\\\cmidrule(lr){2-4}
%     & \google-Sent. & \reddit-Sent. & \reddit-Sarc.\\\midrule[\heavyrulewidth]
%     en-AU & 0.94 & 0.78 & 0.62\\
%     en-IN & 0.64 & 0.69 & 0.56\\
%     en-UK & 0.86 & 0.78 & 0.58 \\\hdashline
%     $\bar{\mu}$ & 0.81 & 0.75 & 0.59\\
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Performance comparison of models based on architecture and training data. The table reports the F1 scores for sentiment and sarcasm classification across three English varieties. Models are grouped by properties: encoder vs. decoder and monolingual vs. multilingual. $\bar{L}$ denotes the average task performance across all locales. $\bar{P}$ denotes the average task performance across all model properties.}
%     \label{tab:arch}
% \end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{adjustbox}{width=1.0\linewidth,center}
%     \renewcommand{\arraystretch}{1}
%     \setlength{\cmidrulekern}{0.25em}    
%     \begin{tabular}{cccccccc}
%     \toprule
%     \multirow{2}{4em}{\centering Locale} & \multicolumn{3}{c}{Domain-Task} & \multicolumn{4}{c}{Model Property} \\\cmidrule(lr){2-4}\cmidrule(lr){5-8}
%     & \google-Sent. & \reddit-Sent. & \reddit-Sarc. & Enc. & Dec. & Mono. & Multi.\\\midrule[\heavyrulewidth]
%     en-AU & 0.94 & 0.78 & 0.62 & 0.79 & 0.77 & 0.78 & 0.78\\
%     en-IN & 0.64 & 0.69 & 0.56 & 0.66 & 0.57 & 0.63 & 0.63\\
%     en-UK & 0.86 & 0.78 & 0.58 & 0.77 & 0.68 & 0.75 & 0.73\\\hdashline
%     $\bar{\mu}$ & 0.81 & 0.75 & 0.59 & 0.74 & 0.67 & 0.72 & 0.71\\
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Performance comparison of models based on architecture and training data. The table reports the F1 scores for sentiment and sarcasm classification across three English varieties. Models are grouped by properties: encoder vs. decoder and monolingual vs. multilingual. $\bar{L}$ denotes the average task performance across all locales. $\bar{P}$ denotes the average task performance across all model properties.}
%     \label{tab:arch}
% \end{table*}

\begin{table*}[t!]
    \centering
    \renewcommand{\arraystretch}{1.1}
    \setlength{\cmidrulekern}{0.25em}    
    \begin{tabular}{p{4em}cccccccccccc}
    \toprule
    \multirow{2}{4em}{Model Property} & \multicolumn{4}{c}{\google-Sentiment} & \multicolumn{4}{c}{\reddit-Sentiment} & \multicolumn{4}{c}{\reddit-Sarcasm}\\\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
    & en-AU & en-IN & en-UK & $\bar{L}$ & en-AU & en-IN & en-UK & $\bar{L}$ & en-AU & en-IN & en-UK & $\bar{L}$\\\midrule[\heavyrulewidth]
    N/A & 0.94 & 0.64 & 0.86 & 0.81 & 0.78 & 0.69 & 0.78 & 0.75 & 0.62 & 0.56 & 0.58 & 0.59\\\hdashline
    Encoder & 0.93 & 0.72 & 0.93 & 0.86 & 0.76 & 0.69 & 0.79 & 0.75 & 0.67 & 0.57 & 0.57 & 0.60\\
    Decoder & 0.96 & 0.48 & 0.71 & 0.72 & 0.83 & 0.68 & 0.75 & 0.75 & 0.52 & 0.54 & 0.59 & 0.55\\\hdashline
    Mono & 0.94 & 0.69 & 0.94 & 0.86 & 0.83 & 0.64 & 0.73 & 0.73 & 0.56 & 0.56 & 0.58 & 0.56\\
    Multi & 0.94 & 0.60 & 0.79 & 0.78 & 0.74 & 0.73 & 0.82 & 0.76 & 0.67 & 0.56 & 0.58 & 0.60\\
    \bottomrule
    \end{tabular}
    \caption{Performance comparison of models based on architecture and training data. The table reports the F1 scores for sentiment and sarcasm classification across three English varieties. Models are grouped by properties: encoder vs. decoder and monolingual vs. multilingual. $\bar{L}$ denotes the average task performance across all locales. $\bar{P}$ denotes the average task performance across all model properties.}
    \label{tab:arch}
\end{table*}
\subsection{Sentiment vs. Sarcasm}
Due to the absence of sarcasm labels in our annotated Google reviews dataset, sarcasm classification is conducted exclusively on Reddit posts. The results show that sarcasm classification achieves lower performance, with an average F1 score of 0.59 across different locales and models, compared to sentiment classification. This performance gap can be partly attributed to the lack of sarcasm annotations (as shown in Table~\ref{tab:stats}). Additionally, it is important to recognize that detecting sarcasm is inherently more difficult because it often relies not just subtle linguistic cues but also localised contemporary contextual information~\cite{abercrombie-hovy-2016-putting}. \textcolor{red}{Show this using topics?}

\subsection{Google Places vs. Reddit}
We examine the impact of domain on model performances on sentiment classification. Our findings indicate that models perform better on Google reviews, achieving an \f score of 0.81, compared to an \f score of 0.75 on Reddit posts. This difference can be explained by the distinct writing styles of the two sources. Google reviews are generally more formal and informative, while Reddit posts and comments often exhibit a short (as shown in Table~\ref{tab:stats}), conversational tone typical of social media. Additionally, Google reviews tend to focus on well-known locations, such as popular tourist attractions, and are often written by individuals who may not be native speakers of the locale-specific variety of English. In contrast, Reddit posts and comments come from forums frequented by local speakers, which means the language and expressions used are more reflective of the regional variety and cultural nuances. \textcolor{red}{Need to be better}.

\subsection{Model properties}
The results in Table~\ref{tab:arch} describes the model performances (reporting \f), grouped based on their properties. These results indicate a consistent trend where encoder models report higher performance than decoder models across different tasks, training data and locales. This performance gap is expected as encoder architecture is inherently better suited for sequence classification tasks, while decoder architecture is optimized for text generation tasks\textcolor{red}{\cite{???}}. Multilingual models also report a marginally higher performance than monolingual models across different tasks and datasets.\textcolor{red}{Why?}.

\subsection{Cross-variety}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figs/cross-mistral.png}
    \caption{Cross-variety performance analysis of \mistral. The figure compares three different scenarios: pre-trained (PT), in-variety fine-tuning, and cross-variety fine-tuning for sentiment and sarcasm classification across all locales.}
    \label{fig:cross-mistral}
\end{figure*}

We further explore the cross-variety generalisation ability of our best-performing model, \mistral. Figure~\ref{fig:cross-mistral} compares performance of \mistral (the best performing model) across three variants: pre-trained, in-variety fine-tuning, and cross-variety fine-tuning, for both sentiment and sarcasm classification tasks.

For sentiment classification, the pre-trained model variant achieves high \f across both datasets, with the best performance of 0.91 on en-UK and the lowest of 0.76 on the Reddit dataset. Fine-tuning the model improves in-variety performance, with noticeable gains in \f on both datasets. However, cross-variety evaluation remains mostly unaffected, except when the model is fine-tuned on en-UK Reddit data. In this case, performance drops across all varieties, with en-IN experiencing the greatest decline. These results suggest that for sentiment classification, the model’s performance is relatively stable across different varieties of English, indicating that domain-specific data plays a minor role in influencing cross-variety generalisation.

As seen earlier, the model performs significantly worse on sarcasm classification compared to sentiment classification. While in-variety evaluation shows that fine-tuning improves over pre-trained model with substantial increases in \f, it negatively impacts cross-variety generalisation. There is a notable decrease in \f across other varieties when the model is fine-tuned on a specific variety. This supports the idea that sarcasm classification requires the model to grasp locale-specific linguistic and cultural nuances, making generalisation across varieties challenging.

% Encoder models seem to consistently report higher \f than decoder models with \textcolor{red}{average performance gap ranging from 0.04 to 0.06. (4 to 6 points) (Show this in the table somehow)}.
% \textbf{Sentiment classification}\\
% \textbf{Google Dataset}\\
% Decoder models report the best performance with \f of 0.96, when evaluated on en-AU subset. Followed by encoder models with \f of 0.94, when evaluated on en-UK subset. The worst performance is reported by decoder models evaluated on the en-IN subset, with \f of 0.48. On average, encoder models report a higher \f of 0.86 compared to 0.72 reported by decoder models.

% \textbf{Reddit Dataset}\\
% Decoder models report the best performance with \f of 0.83, when evaluated on en-AU subset. Followed by encoder models with \f of 0.80, when evaluated on en-UK subset. The worst performance is reported by decoder models evaluated on the en-IN subset, with \f of 0.68. On average, encoder models report a higher \f of 0.75 compared to 0.71 reported by decoder models.

% \textbf{Sarcasm classification}\\
% % \textbf{Reddit Dataset}\\
% Encoder models report the best performance with \f of 0.67, when evaluated on en-AU subset. Followed by decoder models with \f of 0.59, when evaluated on en-UK subset. The worst performance is reported by decoder models evaluated on the en-IN subset, with \f of 0.54. On average, encoder models report a higher \f of 0.61 compared to 0.55 reported by decoder models.

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=1\linewidth]{figs/enc-dec.png}
%     \caption{Encoder v Decoder}
%     \label{fig:enc-dec}
% \end{figure*}
% \subsection{Monolingual vs. Multilingual}
% \textbf{Sentiment classification}\\
% \textbf{Google Dataset}\\
% Both type of models report the best performance with \f of 0.94, when evaluated on en-AU subset. Followed by monolingual models with \f of 0.94, when evaluated on en-UK subset. The worst performance is reported by multilingual models evaluated on the en-IN subset, with \f of 0.60. On average, monolingual models report a higher \f of 0.86 compared to 0.78 reported by multilingual models.

% \textbf{Reddit Dataset}\\
% Monolingual models report the best performance with \f of 0.83, when evaluated on en-AU subset. Followed by multilingual models with \f of 0.82, when evaluated on en-UK subset. The worst performance is reported by monolingual models evaluated on the en-IN subset, with \f of 0.64. On average, multilingual models report a higher \f of 0.76 compared to 0.74 reported by monolingual models.

% \textbf{Sarcasm classification}\\
% % \textbf{Reddit Dataset}\\
% Multilingual models report the best performance with \f of 0.67, when evaluated on en-AU subset. Followed by multilingual models with \f of 0.59, when evaluated on en-UK subset. The worst performance is reported by both type of models evaluated on the en-IN subset, with \f of 0.56. On average, multilingual models report a higher \f of 0.60 compared to 0.57 reported by monolingual models.

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=1\linewidth]{figs/mono-multi.png}
%     \caption{Monolingual v Multilingual}
%     \label{fig:mono-multi}
% \end{figure*}
% \subsection{Augmented Data}
% \subsection{Balanced labels}
